TrackThinkDashboard: Understanding Student Self-Regulated Learning in Programming Study

In programming education, fostering self-regulated learning (SRL) skills is essential for both students and teachers. This paper introduces TrackThinkDashboard, an application designed to visualize the learning workflow by integrating web browsing and programming logs into one unified view. The system aims to (1) help students monitor and reflect on their problem-solving processes, identify knowledge gaps, and cultivate effective SRL strategies; and (2) enable teachers to identify at-risk learners more effectively and provide targeted, data-driven guidance. We conducted a study with 33 participants (32 male, 1 female) from Japanese universities, including individuals with and without prior programming experience, to explore differences in web browsing and coding patterns. The dashboards revealed multiple learning approaches, such as trial-and-error and trial-and-search methods, and highlighted how domain knowledge influenced the overall activity flow. We discuss how this visualization tool can be used continuously or in one-off experiments, consider associated privacy implications, and explore opportunities for expanding data sources to gain richer behavioral insights.

==> Authors/1_introduction.tex <==
\section{Introduction}
\label{section:Introduction}
Programming education has emerged as a vital component of modern professional skill development. To meet the demands of an increasingly technology-driven world, educators must provide hands-on learning experiences that nurture students' self-regulated learning (SRL) skills~\cite{zimmerman2001self}. SRL empowers learners to take charge of their educational journey through goal setting, self-monitoring, reflection, and refinement, ultimately enhancing both academic performance and long-term knowledge retention.

\begin{figure*}[t] 
  \centering 
  \includegraphics[width=1.0\columnwidth]{Authors/figures/proposal.pdf} 
  \caption{Overall workflow of \textit{TrackThinkDashboard}.} 
  \label{fig:workflow_process_trackthink_dashboard} 
\end{figure*}

To enhance SRL in programming education, we present the \textit{TrackThink Dashboard}, an innovative application designed to visualize SRL activity behaviors. The application aims to empower students and teachers by integrating web browsing and programming activities into a unified view. This integration allows users to analyze behaviors such as information searching, resource selection, coding actions, and iterative refinements in learning strategies. By tracking and displaying these activities, the application helps students gain deeper insights into their learning workflows and decision-making processes, fostering a more self-aware and practical approach to learning.

While previous systems like SearchBar~\cite{Morris2008}, popHistory~\cite{Carrasco2017}, and TrackThinkTS~\cite{makhlouf2022} have focused on collecting web browsing logs, and tools such as Log++~\cite{marron2018} and Projection Boxes~\cite{Lerner2020} have captured programming activity logs, these studies have not addressed the integration and classification of behaviors across both domains. Our approach bridges this gap by recognizing and visualizing the flow of web browsing and programming activities as an integrated process.

The application enables students to analyze their activity behaviors, such as transitions between web searches and coding tasks. Students can identify knowledge gaps, optimize resource usage, and refine learning strategies by visualizing these behaviors over time. This metacognitive~\cite{watanabe2024metacognition} awareness fosters the development of a more structured and effective learning process.
The dashboard provides teachers with detailed insights into students' activity patterns and challenges, supporting targeted and data-driven interventions. 

Through activity recognition, teachers can classify behaviors such as prolonged resource searching, recurring coding errors, or inefficient task-switching, allowing them to identify students who may need additional guidance. Furthermore, the platform facilitates collaboration between students and teachers by encouraging discussions around specific behaviors and strategies, enhancing the overall learning experience.

This paper proposes an application that leverages web browsing and programming activities to visualize students' SRL workflow in programming learning. As shown in Figure~\ref{fig:workflow_process_trackthink_dashboard}, we use a web browsing activity logger~\cite{makhlouf2022} and a programming IDE~\cite{C2Room} to collect logs. The \textit{TrackThink Dashboard} synchronously visualizes two activities, offering an intuitive GUI (Graphical User Interface) that allows users to visualize their activities as a structured flowchart. Our contributions are as follows: 

\begin{enumerate} 
  \item \textbf{A unified visualization of web browsing and programming}: We introduce an application that combines web browsing and programming activities as an all-in-one flowchart.
  \item \textbf{We discover the pattern of SRL behavior through web browsing and programming activity}: Using our application, we identify how students transition between web browsing and programming tasks, revealing an understanding of the patterns of SRL workflow.
\end{enumerate}

==> Authors/2_related_literature.tex <==
\section{Related Work}
In this section, we explain related work regarding the data collection tools for web browsing and programming. We will also show a sample visualization analysis using web browsing and programming logs, with some highlighted examples.

\subsection{Web Browsing Activity Log Collection}
Several tools have been developed to log and analyze web browsing activities. Mermite~\cite{wong2007} lets users store multiple web resources and create mashups without needing programming skills. Users can organize content, like flight prices or publication years, in any order. SearchBar~\cite{Morris2008} saves browsing and query histories along with user ratings and notes, making it easier to highlight important actions, such as favorite websites or frequently used queries. This approach helps users visualize their browsing behavior and even share patterns with others. PopHistory~\cite{Carrasco2017} presents web history as a bubble chart, where bubble sizes indicate frequently visited sites. LogCanvas~\cite{xu2018} collects web search histories and visualizes them as knowledge graphs, helping users see connections between pages rather than simply listing URLs. Lastly, TrackThinkTS~\cite{makhlouf2022, watanabe2023trackthink} is a browser extension inspired by TrackThink~\cite{nagano2017}. It logs tab and window operations with timestamps and exports data in CSV format, simplifying log analysis. These tools underscore the value of web browsing logs for both personal and shared insights.

\subsection{Programming Activity Log Collection}
Several tools have been developed to log and analyze programming activities. Log++~\cite{marron2018} captures logging results in JSON format, focusing on optimizing logging statements rather than recording compilation histories or results. Projection Boxes~\cite{Lerner2020} provides a summary of compilation results and timestamps, displaying code statements in a box format, but it’s not designed to collect detailed compile logs. C2Room~\cite{C2Room} is an online programming IDE that logs timestamps, compiled code, and results. It also allows users to set programming tasks, recording task IDs and timestamps, making it easy to track code progress and outcomes. Similarly, WEVL~\cite{su14138084} supports online programming environments with comparable functionality. Lastly, Log-it~\cite{Jiang2023} is a Visual Studio Code extension that visualizes programming workflows, enabling users to easily reference historical code patterns through its visual interface.

\subsection{Visualize Web Browsing and Programming}
The integration of web browsing and programming logs has drawn attention in recent research to better understand data interactions. Prompter~\cite{ponzanelli2016} is an IDE plugin that retrieves relevant Stack Overflow discussions, ranks their relevance using a multifaceted model, and displays them to developers within the Eclipse IDE. A study involving 33 developers reported a 74\% positive response rate. This concept was later expanded in Libra~\cite{ponzanelli2017}, which provides comprehensive web resource recommendations directly within the IDE. CrossRec~\cite{phuong2020} recommends third-party libraries by analyzing attached code. \citeauthor{brandt2009two} explored how developers use online resources for technical problem-solving~\cite{brandt2009two}, revealing that programmers engage in \textit{just-in-time} learning and use online materials for both acquiring new skills and clarifying existing knowledge. Additionally, \citeauthor{watanabe2022} investigated the estimation of programming domain knowledge from web and programming log data~\cite{watanabe2022}. By categorizing participants as domain experts or novices, the study achieved a prediction accuracy of 0.95 using Random Forest, highlighting significant behavioral differences between novice and expert programmers in web browsing and coding.

In summary, while existing works provide valuable insights into integrating web browsing and programming logs, none offer a clear visualization of the learning path in programming.

==> Authors/3_method.tex <==
% \begin{figure}[t]
%   \centering
%   \includegraphics[width=0.65\columnwidth]{Authors/figures/system_flow.pdf}
%   \caption{System Architecture. Data sources are reshaped and filtered prior to visualization. The visualization shows flow-chart and pie-chart.}
%   \label{fig:system-overview}
% \end{figure}

\section{Methodology}
\label{section:methodology}
We use two applications for logging web browsing and programming activity to visualize both activities synchronously. This section explains data source, fusion, and visualization approaches for understanding SRL.

\subsection{Data Source}
\label{section:data_source}
In this section, we explain the data source. In our prior study, we aim to use web browsing and programming logs. We use the web browser logger TrackThinkTS~\cite{makhlouf2022} and C2Room~\cite{C2Room}, an online programming IDE for collecting programming activity logs. We will explain web browsing and programming logs in detail.

% \begin{table}[t!]
%   \centering
%   \caption{Web browsing log collected by TrackThinkTS.}
%   \renewcommand{\arraystretch}{1.0}
%   \small
%   \begin{tabular}{l p{5.0cm}}\hline
%     Column Name                  & Description \\ \hline
%     UserID                       & Participant's user ID. \\
%     UserAction                   & User action (e.g., tab, scroll, copy). \\
%     date                         & Log timestamp in UNIXTIME. \\
%     Tab\_URL                     & URL of the accessed page. \\
%     Tab\_Title                   & Title of the accessed page. \\
%     Tab\_BodyText                & Body text of the accessed page. \\
%     ClipboardCopy                & Copied text content. \\
%     Scroll\_YAxisSpeed           & Vertical scroll speed. \\
%     Scroll\_VisibleText          & Visible text after scroll. \\
%     Scroll\_ViewPort\_XScroll    & Horizontal scroll viewport. \\
%     Scroll\_ViewPort\_YScroll    & Vertical scroll viewport. \\
%     Scroll\_XScrollRate          & Horizontal scroll percentage. \\
%     Scroll\_YScrollRate          & Vertical scroll percentage. \\
%     ViewPortWidth                & Viewport width. \\
%     ViewPortHeight               & Viewport height. \\
%     DocWidth                     & Document width. \\
%     DocHeight                    & Document height. \\ \hline
%   \end{tabular}
% \label{tab:table_trackthinkts}
% \end{table}

Web browsing activities are recorded through a web browser extension called TrackThinkTS~\cite{makhlouf2022}, designed to prioritize user privacy. One notable advantage of TrackThinkTS over other web browser loggers is its user-friendly interface, allowing participants to delete irrelevant logs collected during the experiment. Users need to install this extension in their web browser to utilize it. In our study, we have selected Google Chrome~\footnote{\url{https://www.google.com/chrome/}} as the preferred web browser.

Programming activities are recorded through an online web IDE called C2Room~\cite{C2Room}. The application is tailored for online programming classes in educational institutions and companies. The log lets us understand how and when users execute their code in the compiler and the compiled result. The application also allows users to track when they are satisfied with their written code and proceed to submit it.

\begin{table}[t!]
  \centering
  \caption{Selected log after from TrackThinkTS~\cite{makhlouf2022} and C2Room~\cite{C2Room}.}
  \renewcommand{\arraystretch}{1.0}
  \small
  \begin{tabular}{l p{6.5cm}}\hline
    Column Name   & Description \\ \hline
    timestamp     & Time of the action in UNIXTIME. \\
    userID        & Participant ID during SRL. \\
    taskID        & Task/question ID created by the organizer. \\
    userAction    & Action logs collected from data sources. \\
    tabURL        & URL of the accessed web page. \\
    clipboardCopy & Text copied to the clipboard. \\
    msg           & Compile message (e.g., status, output, errors). \\ \hline
  \end{tabular}
\label{tab:table_data_fusion}
\end{table}

% \begin{table}[t!]
%   \centering
%   \caption{Elements of user actions after data fusion.}
%   \renewcommand{\arraystretch}{1.0}
%   \small
%   \begin{tabular}{l p{4.5cm}}\hline
%     User Action      & Description \\ \hline
%     Tab creation     & Opening a new tab. \\
%     Tab activation   & Selecting an existing tab. \\
%     Tab refresh      & Reloading in the same tab. \\
%     Tab remove       & Deleting a tab. \\
%     Clipboard copy   & Copying text to the clipboard. \\
%     Start compiling  & Starting code compilation. \\
%     End compiling    & Ending code compilation. \\
%     Submit code      & Submitting code. \\ \hline
%   \end{tabular}
% \label{tab:table_user_action_after_data_fusion}
% \end{table}

\subsection{Data Fusion}
\label{section:data_fusion}
Data fusion is applied to the collected data sources. The data fusion process comprises two primary procedures: data shaping and filtering. Data shaping involves transforming raw data into a unified format suitable for combining various data sources. Data filtering entails selecting relevant data points following the conversion and concatenation. These processes are crucial in simplifying the visualization, enabling students and teachers to comprehend the performance metrics easily during SRL in programming. We will now provide a detailed explanation of each procedure.

We employ data shaping as a preprocessing step to facilitate the concatenation and filtering of logs. We rename the columns for each web browsing and programming log. Specifically, we begin by renaming the columns \textit{date} and \textit{time} to \textit{timestamp}. Additionally, we rename \textit{UserID} and \textit{uid} to \textit{userID}. For \textit{UserAction} and \textit{op}, we change to \textit{userAction}. Once the column renaming is complete, we convert the \textit{timestamp} values to UNIXTIME and sort them chronologically.

Table~\ref{tab:table_data_fusion} shows the table after data filtering. Some information is removed, such as window scroll speed from the web browsing log, class ID from the programming log, or logs involving NAN values. In order to sort logs into time order, we convert all units of the timestamp into UNIXTIME. Specifically, the programming logs collected by C2Room were converted from JST to UNIXTIME. All the logs are concatenated and sorted in a time order using \textit{timestamp}.

\subsection{Visualization}
\label{section:visualization}
Visualization of web browsing and programming activity is performed after data fusion. Figure~\ref{fig:visualization} shows the library used for visualization. For the visualization, we choose a flowchart and pie-chart. We will explain the implementation process and the reason for the choice in detail.

The flowchart is selected to visualize the problem-solving progress in a time series. The approach uses flowcharts to understand what search results participants used to arrive at their answers and what compilation errors they encountered when re-running their searches. The flowchart is implemented using \textit{flowchart.js}~\cite{flowchartjs}. It is a JavaScript library for flowchart SVG (Scalable Vector Graphics) rendering that runs in the terminal and browser. We categorize users' activities in different colors and shapes for start and stop edges.
The workflow is not visualized fully on the screen, but the user can scroll horizontally to see the actions between the start and end edges. For edges like \textit{tab activate} or \textit{tab update}, the hyperlink is set so that users can jump to the webpage once they tap the edge.

\begin{figure*}[t]
  \centering
  \begin{minipage}[t]{0.6\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{Authors/figures/visualization.pdf}
    \caption{Application workflow. Visualization of flowchart and pie-chart.}
    \label{fig:visualization}
  \end{minipage}
  \hfill
  \begin{minipage}[t]{0.35\textwidth}
    \centering
    \includegraphics[width=1.0\linewidth]{Authors/figures/experimental_setting.png}
    \caption{Experimental settings. Collect logs while solving scheme questions.}
    \label{fig:experimental-settings}
  \end{minipage}
\end{figure*}

The pie-chart is selected for visualization because the activity ratio of user action is essential in identifying users' domain knowledge~\cite{watanabe2022}. The pie chart is implemented using \textit{chart.js}~\cite{da2019learn}. Clicking each element removes a specific activity from the pie chart. This option helps teachers or students focus on the ratio of an activity they want to compare. It is a JavaScript library for making HTML-based charts.


==> Authors/4_dataset.tex <==
\section{Data Collection}
\label{section:data_collection}

\subsection{Participants}
In this experiment, we collect logs from lecture students (Dataset A) and non-lecture students (Dataset B). The total number of participants is 33 unique (32 males and one female) university students in Japan.

Dataset A -- University students attending lectures: We collect data from 13 unique university students (12 males and one female) in Japan. Participants have taken university courses in Scheme programming language, so they have knowledge on Scheme grammar or syntax.

Dataset B -- University students not attending lectures: We collected data from 20 male university students in Japan. Participants did not take any university courses related to the Scheme, so they do not have any knowledge from the class, such as Scheme grammar or syntax.

\subsection{\textbf{Experiment Procedure}}
Figure~\ref{fig:experimental-settings} shows the condition of the experiment. Before the experiment, \textit{C2Room} and \textit{TrackThinkTS} were installed on each participant's laptop. Under these conditions, the experiment was conducted using the following procedure: (1) The experiment conductor presents the purpose of the experiment, experimental conditions, and tools that will be provided to the participant. Only the person who agrees with the conditions can participate in the experiment. (2) The participant enters the personal workstation and starts web browsing and programming loggers. (3) Participants work on solving problems with a given schema using the \textit{C2Room} programming editor. The order of question-solving is not restricted, but it is assumed that the participant will solve the easy questions step by step. \textit{C2Room} will record the compiled results for each question. (4) Participants may use a web search engine to find the answer. \textit{TrackThinkTS} will track web browsing behavior. (5) The participant submits the answer and moves on to the next question when satisfied with the code compilation. Allow the student to return to previous questions to change the answer. (6) When all questions have been answered or an hour has passed, we stop participants from problem-solving. (7) Participants remove privacy-sensitive logs from \textit{TrackThinkTS}. Once all recorded logs are submitted to the experimenter, the participant leaves the personal workspace.

In this study, we recruit the same Scheme questions as \citet{watanabe2022}. We have prepared ten questions in order of difficulty. Easy questions are those that require fewer lines of code to solve. In this experiment, we chose Scheme (Racket), one of the dialects of LISP languages, as the programming language of the task~\cite{adams1995}. We chose this task because of its simple language specification, used in programming courses at several universities. Also, it is tailored for lecture use, so its language specification is usually unknown to students except those attending the lecture.

==> Authors/5_result.tex <==
\section{Result}
In this section, we show results obtained from the \textit{TrackThink Dashboard}.

Figure~\ref{fig:try_and_error_group} shows a sample student workflow for solving a programming problem using the try-and-error approach. Students compile the code, and after receiving an error response, they modify it and try to recompile it. Some students do a try-and-error flow more than twice before returning to the web browser to find an answer.

Figure~\ref{fig:try_and_search_group} shows an example student working on the same task and receiving an error response, but this user decides to go back to the web search before the following compilation.
We call this pattern of solving a try-and-search student. The student copies the error message from the compiler and inserts and searches in the web browser. Both students receive an error response on the same problem, but each student acts differently to continue solving the problem.

Figure~\ref{fig:cautios_group} illustrates a sample workflow of a student group tackling a programming task. A defining characteristic of these students is their approach of first gathering information from web pages before attempting to solve the problem. Once they have a clear understanding of the solution, they return to the online IDE to code and submit their work. While two students in this group follow similar workflows, one writes the code from scratch, whereas the other copies sections of code using the clipboard. Both demonstrate a methodical approach, prioritizing understanding over immediate action. We refer to this group as \textit{cautious students}.

\begin{figure}[t!]
  \centering
  \captionsetup[subfigure]{justification=centering}
  \subfloat[\textit{Student A} receives an error response and retry until compilation success.]{
    \includegraphics[width=0.48\columnwidth]{Authors/figures/wf_try_and_error_rush.png}
  }
  \hfill
  \subfloat[\textit{Student B} receives an error response and retries compile once more.]{
    \includegraphics[width=0.48\columnwidth]{Authors/figures/wf_try_and_error.png}
  }
  \hfill
  \caption{Group of try-and-error students. Students receive an error response after compiling, and students try to compile before going back to the web search.}
  \label{fig:try_and_error_group}
\end{figure}

\begin{figure}[t!]
  \centering
  \captionsetup[subfigure]{justification=centering}
  \subfloat[\textit{Student C} receives an error and goes back to search on the web.]{
    \includegraphics[width=0.48\columnwidth]{Authors/figures/wf_try_and_search.png}
  }
  \hfill
  \subfloat[\textit{Student D} receives an error and goes back to search on the web.]{
    \includegraphics[width=0.48\columnwidth]{Authors/figures/wf_try_and_search_2.png}
  }
  \hfill
  \caption{Group of try-and-search students. Students receive an error response after compiling, and students return to the web browsing to find a solution before the following compilation.}
  \label{fig:try_and_search_group}
\end{figure}

\begin{figure}[t!]
  \centering
  \captionsetup[subfigure]{justification=centering}
  \subfloat[\textit{Student E} seek information from webpage and write code.]{
    \includegraphics[width=0.48\columnwidth]{Authors/figures/wf_search_compile.png}
  }
  \hfill
  \subfloat[\textit{Student F} seek information from webpage and use clipboard copy action to submit code.]{
    \includegraphics[width=0.48\columnwidth]{Authors/figures/wf_copy.png}
  }
  \hfill
  \caption{Group of cautious students. Students use web searches before programming. Once the solution is identified, write code from scratch or use a clipboard copy to solve the task.}
  \label{fig:cautios_group}
\end{figure}

\begin{figure}[t!]
  \centering
  \captionsetup[subfigure]{justification=centering}
  \subfloat[\textit{Student G} check few programming tasks after starting experiment.]{
    \includegraphics[width=0.48\columnwidth]{Authors/figures/wf_time_manager.png}
  }
  \hfill
  \subfloat[\textit{Student H} check all programming tasks after starting experiment.]{
    \includegraphics[width=0.48\columnwidth]{Authors/figures/wf_time_manager_2.png}
  }
  \hfill
  \caption{Group of time management students. Students move to other tasks after starting problem-solving. One participant look for a few questions, whereas the other student look at all questions before starting to solve questions.}
  \label{fig:time_manager_group}
\end{figure}

\begin{figure}[t!]
  \centering
  \captionsetup[subfigure]{justification=centering}
  \subfloat[\textit{Student I} submit code in the last moment of the experiment.]{
    \includegraphics[width=0.48\columnwidth]{Authors/figures/wf_double_check.png}
  }
  \hfill
  \subfloat[\textit{Student J} submit code in the last moment of the experiment.]{
    \includegraphics[width=0.48\columnwidth]{Authors/figures/wf_double_check_2.png}
  }
  \hfill
  \caption{Group of double checking students. Students move to previous questions to double check and submit their code before finishing the experiment.}
  \label{fig:double_check_group}
\end{figure}

\begin{figure}[t!]
  \centering
  \captionsetup[subfigure]{justification=centering}
  \subfloat[Sample pie-chart for non-lecture attendee student]{
    \includegraphics[width=0.3\columnwidth]{Authors/figures/pie_novice_web}  
    \hspace{1mm}
    \includegraphics[width=0.3\columnwidth]{Authors/figures/pie_novice_compile.png}
    \hspace{1mm}
    \includegraphics[width=0.3\columnwidth]{Authors/figures/pie_novice_all.png}
  }
  \hfill
  \subfloat[Sample pie-chart for lecture attendee student]{
    \includegraphics[width=0.3\columnwidth]{Authors/figures/pie_expert_web}  
    \hspace{1mm}
    \includegraphics[width=0.3\columnwidth]{Authors/figures/pie_expert_compile.png}
    \hspace{1mm}
    \includegraphics[width=0.3\columnwidth]{Authors/figures/pie_expert_all.png}
  }
  \hfill
  \caption{Pie-chart of selected non-lecture and lecture attendance students. The pie-chart represents a ratio of students' action counts. The left shows an action ratio of web browsing logs, the middle shows the ratio of programming compilation result counts, and the right shows the ratio of all action counts.}
  \label{fig:pie_chart}
\end{figure}

Figure~\ref{fig:time_manager_group} presents an example workflow of students who strategically review multiple questions at the start of the experiment. While one student examines only a few questions, another reviews all of them before beginning their solutions. Notably, this behavior was absent among non-lecture students and was exclusive to lecture attendees, who possess domain knowledge of the programming language. These students prioritize solving easier questions first, optimizing their time and effort. We refer to this group as \textit{time management students}.

Figure~\ref{fig:double_check_group} shows a workflow typical of the \textit{double-checking students} group. Before concluding the experiment, these students revisit all programming questions to carefully review their submissions. This behavior reflects their thorough and detail-oriented problem-solving approach.

Finally, Figure~\ref{fig:pie_chart} displays action ratio pie charts from the experiment, comparing non-lecture and lecture attendees. The pie charts illustrate the proportion of time spent on web browsing, programming, and a combination of the two. Students who attended lectures, possessing greater domain knowledge, exhibited a higher success rate in code compilation compared to errors. Conversely, non-lecture students experienced more compilation errors and relied more heavily on web searches. These differences align with findings from prior research~\cite{watanabe2022}.


==> Authors/6_limitation.tex <==
\section{Discussion and Future Work}
\label{section:discussion_future_work}
Our study visualizes a flowchart by combining web browsing and programming data to understand students' self-regulated learning (SRL) workflows. This approach provides insights into how students tackle each task, analyzing their learning activities while uncovering individual differences. Flowcharts capture detailed problem-solving processes, while pie charts highlight frequently used actions, offering a clearer understanding of programming language comprehension~\cite{watanabe2022}. Pie charts help monitor problem-solving progress, while flowcharts enable a closer examination of the steps students take, shedding light on their thought processes and strategies.

Although effective, the current visualization has limitations. One limitation is the lack of action duration representation. Actions are sorted by timestamps, but varying node lengths to reflect duration could help identify when students encounter difficulties. The flowchart could also be enhanced by separating actions into branches, such as web browsing and programming, inspired by Git’s branching system~\cite{chacon2014pro}. While the current single-line design is simpler, branching could reveal more nuanced workflows in some contexts.

Integrating additional sensor data offers another improvement opportunity. Potential plugins include wearable devices to monitor physiological data for measure stress~\cite{garg2021stress} or fatigue~\cite{ElsenRonando202418}, eye-tracking~\cite{AnkurBhatt20249} to measure attention~\cite{ishimaru2016towards} or concentration~\cite{SakiTanaka202410}, facial recognition technology to assess micro-behaviors or engagement levels~\cite{watanabe2021discaas, watanabe2023engauge}, and bluetooth based position estimation~\cite{bello2024besound}. Such data could provide deeper insights into students’ cognitive states and behaviors.

Our analysis identified five SRL patterns during web browsing and programming: \textit{try and error}, \textit{try and search}, \textit{cautious}, \textit{time management}, and \textit{double checking}. Combining knowledge input (web browsing) with knowledge output (programming) revealed unique problem-solving approaches that submitted code alone cannot capture. These insights help teachers understand students better and guide their coaching. Additionally, the dashboard highlights high-performing students' workflows, offering a resource for novice learners. Pie charts also reveal domain knowledge~\cite{watanabe2022}.

Finally, several limitations remain. Current analysis focuses on individual patterns without considering combinations, such as \textit{cautious} students also using \textit{time management} strategies. Exploring such combinations could provide a better understanding of problem-solving processes. The programming tasks used in this study were relatively simple, focusing on Scheme syntax, leading to limited score variability. Future work should design tasks that encourage diverse strategies and performance levels.

% Finally, our study focuses on traditional web browsing activities during programming. Future work will integrate interactions with GPT-based tools like ChatGPT~\cite{chatGPT2022}. By logging prompts and analyzing how students use tools like ChatGPT, we aim to understand their problem-solving processes better. This expansion will broaden our understanding of web browsing and AI-assisted workflows in programming.


==> Authors/7_conclusion.tex <==
\section{Conclusion}
\label{section:conclusion}
In this paper, we presented the \textit{TrackThink Dashboard}, a system designed to visualize SRL workflows through flowcharts and pie charts based on web browsing and programming activity logs. Using data collected from 33 university students solving tasks in the Scheme programming language, the visualization revealed distinct and unique problem-solving patterns. This research offers valuable insights into the SRL process, enabling students to refine their learning strategies and providing teachers with actionable feedback to enhance study efficiency and support individualized learning.
